ACE: Concept Editing in Diffusion Models without Performance Degradation

Diffusion-based text-to-image models have demonstrated remarkable capabilities in generating realistic images, but they raise societal and ethical concerns, such as the creation of unsafe content. While concept editing is proposed to address these issues, they often struggle to balance the removal of unsafe concept with maintaining the model's general genera-tive capabilities. In this work, we propose ACE, a new editing method that enhances concept editing in diffusion models. ACE introduces a novel cross null-space projection approach to precisely erase unsafe concept while maintaining the model's ability to generate high-quality, semantically consistent images. Extensive experiments demonstrate that ACE significantly outperforms the advancing baselines,improving semantic consistency by 24.56% and image generation quality by 34.82% on average with only 1% of the time cost. These results highlight the practical utility of concept editing by mitigating its potential risks, paving the way for broader applications in the field. Code is avaliable at https://github.com/littlelittlenine/ACE-zero.git

==> chapters/2related.tex <==
\section{Related Work}
\textbf{Unsafe Concepts in T2I Models.} T2I models can inadvertently generate unsafe images such as nude, violent, and copyright infringing imagery \cite{extracted_concept,extracted_concept_2}. Additionally, another risk of T2I models is the internalization and amplification of social and cultural biases within diffusion models \cite{bias_1,bias_2,bias_3}, since the stereotypes inherent in the training data could be reflected and reinforced in the T2I models. 

Previous approaches to address unsafe issues in diffusion models have proposed several strategies, categorized as follows: First, filtering the training data and retraining the model. However, this method is resource-intensive and unpredictable, as even seemingly benign data may lead to unsafe outputs. Second, Safety checkers \cite{red} and Non-classifier Guidance \cite{safe_guide，}, Implementing safety checkers or integrating non-classifier guidance during inference seeks to prevent the generation of unsafe content. These measures, however, can be easily circumvented in open-source settings. Third, Parameter Fine-tuning \cite{ESD,Ablation}, which involves adjusting the parameters of pre-trained models to limit unwanted performance. While potentially effective, this approach incurs significant computational costs.  

\vspace{5pt}
\noindent\textbf{Closed-form Editing for T2I Models.} Recent advancements in closed-form editing have shown promise in effectively erasing unsafe concepts \cite{UCE,RECE}, ensuring compliance while minimizing the risk of circumvention. Specifically, these methods focus on editing pre-trained model parameters to specifically target and erase outputs related to violating concepts, showing notable efficiency in preventing undesirable content generation. However, current paradigm faces a critical trade-off: (1) erasing unsafe concepts often compromises (2) the preservation of normal concepts. Ensuring safe outputs results in distorted normal text representations, degrading the model’s general generative capabilities.
Drawing inspiration from null space editing in large language models \cite{null_space,alphaedit}, our approach leverages a balance between knowledge preservation and modification, effectively editing unsafe concepts and enhancing both model performance and fairness.


==> chapters/2related_old.tex <==
\section{Related Work}
\textbf{Unsafe Concepts in T2I Models.} T2I models can inadvertently generate unsafe images \cite{extracted_concept,extracted_concept_2}. To address this issue, existing methods employ strategies like training data randomization, title enhancement \cite{caption_auguement}, and image masking to protect original content \cite{image_mask_1,image_mask_2}. However, they necessitate extensive preprocessing of the training dataset, which can be resource-intensive and time-consuming. Additionally, filtering methods, such as safety detectors, are often easily disabled in open-source platforms, reducing their effectiveness.

\vspace{5pt} % 可以选择添加垂直空间

\noindent \textbf{Nudity and Violence in T2I Models.} Similar to copyright issues, existing researches to mitigate this risk involve the use of filtering methods to detect and eliminate inappropriate content. However, these methods can be circumvented, especially in open-source models. Recent advancements in closed-form editing have shown promise in effectively erasing violating concepts \cite{UCE,RECE}, ensuring compliance while minimizing the risk of circumvention.

\vspace{5pt} % 可以选择添加垂直空间

\noindent \textbf{Social Biases in T2I Models.} A significant issue in image generation is the internalization and amplification of social and cultural biases within diffusion models \cite{bias_1} \cite{bias_2} \cite{bias_3}. These models can reflect and reinforce stereotypes inherent in their training data. To combat this, previous studies have explored several mitigation strategies, including parameter adjustments, removal of bias vectors from text embeddings \cite{debias_vl}, and performing algebraic manipulation of the
representations \cite{concept_algebra}. Drawing inspiration from zero-shot editing in large language models \cite{UCE}, our approach leverages a balance between knowledge preservation and modification, effectively reducing bias and enhancing both model performance and fairness.

\vspace{5pt} % 可以选择添加垂直空间

\noindent \textbf{Model Editing for T2I Models.} Previous approaches to address unsafe issues in diffusion models have proposed several strategies, categorized as follows: First, filtering the training data and retraining the model. However, this method is resource-intensive and unpredictable, as even seemingly benign data may lead to unsafe outputs. Second, Safety checkers \cite{red} and Non-classifier Guidance \cite{safe_guide，}, Implementing safety checkers or integrating non-classifier guidance during inference seeks to prevent the generation of unsafe content. These measures, however, can be easily circumvented in open-source settings. Third, Parameter Fine-tuning \cite{ESD} \cite{Ablation}: This strategy involves adjusting the parameters of pre-trained models to limit unwanted performance. While potentially effective, this approach incurs significant computational costs. Fourth, Closed-form Parameter Editing \cite{UCE} \cite{RECE}: This method focuses on editing pre-trained model parameters to specifically target and erase outputs related to violating concepts, showing notable efficiency in preventing undesirable content generation. 


==> chapters/3method_old.tex <==
\section{Preliminary}
Diffusion Models
Diffusion models have recently achieved remarkable success in generating high-quality images. These models iteratively refine a noisy initial state 
x
T
x 
T
​
  (random noise) into a clear image 
x
0
x 
0
​
  by progressively denoising the input at each timestep 
t
t. Specifically, at each intermediate step, the model predicts and removes a small amount of noise 
ϵ
t
ϵ 
t
​
  from the current image state. This denoising process can be formulated as a Markov chain:

For text-to-image generation, diffusion models often integrate text embeddings (e.g., from CLIP) into their cross-attention modules. These modules use a query-key-value architecture, where image features serve as queries, and text embeddings are transformed into keys and values via attention matrices 
W
k
W 
k
​
  and 
W
q
W 
q
​
 . This enables effective interaction between image and text representations.
The stable diffusion model introduces a novel method for simulating probability distributions by progressively transforming random noise into clear images, a foundational concept in stable diffusion. This process involves a series of fine iterative steps that reduce noise, starting from an initial random state and culminating in a coherent image representation. At each intermediate stage ($t$), the model predicts and adds a small amount of noise ($\epsilon_t$) to the current image state, beginning with random noise ($x_T$) and aiming to produce a clear image ($x_0$) after several denoising iterations. This denoising trajectory can be effectively modeled as a Markov process, and by training the model on the parameters governing this process, we can "sculpt" new images from random noise.

\begin{equation}
p_\theta(x_{T:0}) = p(x_T) \prod_{t=T}^1 p_\theta(x_{t-1} | x_t)
\end{equation}

In the context of text-to-image generation, the stable diffusion model operates within a low-dimensional space, utilizing a U-Net architecture for denoising and image synthesis. Text is encoded using language models such as CLIP, and its guiding influence is incorporated into the U-Net through a cross-attention mechanism. This cross-attention module employs a query-key-value (QKV) architecture, 
\begin{equation}
A \propto \text{softmax}\left(q_i k_i^T\right)
\end{equation}where image features act as the queries and text embeddings are transformed into keys and values. The keys, representing text features, are computed to derive attention scores by multiplying them with the query representations of visual features ($q_i$), thereby revealing the correlations between text tokens and image features. The resulting value vectors of the text features are then weighted and aggregated based on the attention scores, facilitating interaction between visual and textual information.

The Unbiased Cross-Editing (UCE) method provides a fresh perspective on adjusting violating concepts and biases in pre-trained models. By modifying the projection matrices ($W_k$) and ($W_v$) in the cross-attention layer, we can recalibrate the embedding relationships between source and target prompts, enabling precise editing of specific concepts.

The UCE objective minimizes a loss function that accounts for the difference between the edited and target embeddings, alongside changes in the model. 
\begin{equation}
% \small
\min_{W} \sum_{c_i \in E} \left\| W c_i {-} v_i^* \right\|_2^2 {+}\! \sum_{c_j \in P} \left\| W c_j {-} W_{old} c_j \right\|_2^2
\end{equation}
Leveraging a closed-form solution, this editing process can be efficiently executed in under a minute.
\begin{equation}
\small
W{=}\!\left(\sum_{c_i \in E} v_i^* c_i^T \!{+}\!\! \sum_{c_j \in P} W_{old} c_j c_j^T \!\right)\!\!\!\left( \sum_{c_i \in E} c_i c_i^T \!{+}\!\! \sum_{c_j \in P} c_j c_j^T \!\right)^{\!\!{-}1}
\end{equation}
Additionally, UCE incorporates a retention term to preserve relevant concepts, minimizing adverse effects on overall model performance.

However, this editing strategy may inadvertently influence related concepts. To mitigate this issue, we introduce a new retention term that enables precise adjustments to model parameters for specific concept editing while retaining unrelated concepts. This approach enhances the accuracy of the editing process while safeguarding the model's core generative capabilities.

Despite these advancements, the editing strategy faces challenges in balancing knowledge update errors with knowledge retention errors. Excessive emphasis on knowledge updates can lead to overfitting and a decline in the model's original performance during continuous and large-batch editing. To address this, we extract an orthogonal space relative to the retention term (termed zero space), allowing us to project incremental parameter weights into this space. This enables a harmonious balance between model capability retention and concept editing, thereby enhancing editing accuracy while preserving the model's core generative abilities.

\begin{figure}[htp]
    \centering
    \includegraphics[width=8cm]{method.png}
    \caption{\textbf{Null-space constrained cross-attention weight editing.} Our method constructs the null space of preserved concepts ($c_j \in P$) to constrain parameter modifications associated with a specific text embedding of the editing concepts ($c_i \in E$), focusing on their corresponding keys and values within the null space. This approach shifts the dual objective of erasure and preservation to a singular objective of erasure under specific conditions. While maintaining the preserved concepts, we can concentrate on editing the target concepts, facilitating the processes of erasure and debiasing.
}
    \label{fig:galaxy}
\end{figure}

\section{Methodology}
\subsection{Edit in Null-Space}
In this section, we leverage editing techniques from large language models to introduce a zero-space constraint-based approach for editing text-to-image models, with the objective of preserving the integrity of prior knowledge during the editing process. The concept of zero space is defined such that for given matrices ($A$) and ($B$), if ($BA = 0$), then ($B$) resides within the zero space of ($A$). To maintain the knowledge that must be preserved in a lower-dimensional space, we project the perturbation ($\Delta$) onto the left null space of ($K_0$) before incorporating it into the model parameters ($W$). This ensures that the retained knowledge satisfies the condition

\begin{equation}
(W + \Delta) K_0 = W K_0 = V_0.
\end{equation}

To overcome the computational and storage challenges associated with direct projection in the high-dimensional null space of ($K_0$), we adopt the null space of the non-centered covariance matrix ($K_0 K_0^T$) as a feasible alternative. By performing Singular Value Decomposition (SVD), we derive the projection matrix

\begin{equation}
P = U \hat{U}^T.
\end{equation}


which effectively maps perturbations into its null space while ensuring stability of the knowledge through the condition

\begin{equation}
\Delta P K_0 = 0.
\end{equation}


For optimizing the model editing objective, we utilize the projected perturbation ($\Delta P$) in place of the original perturbation, omitting terms associated with ($K_0 K_0$). This leads to the following optimization objective function:


\begin{equation}
\begin{aligned}
\Delta = & \arg \min_{\tilde{\Delta}} \Bigg( |(W + \tilde{\Delta} P) K_1 - V_1|^2 \\
& + |\tilde{\Delta} P|^2 + |\tilde{\Delta} P K_p|^2 \Bigg).
\end{aligned}
\end{equation}



where ($K_1$) and ($V_1$) denote the knowledge key-value matrices to be updated, and ($K_p$) and ($V_p$) represent the previously updated knowledge. By minimizing ($|\tilde{\Delta} P K_p|^2$), we safeguard prior knowledge from disruption. The final perturbation expression is derived through the normal equation solution:

\begin{equation}
\Delta \text{AlphaEdit} = R K_1^T P (K_p K_p^T P + K_1 K_1^T P + I)^{-1}.
\end{equation}


\subsection{Erasure of Artistic Styles and Inappropriate Concepts}
While the Unbiased Cross-Editing (UCE) and Related Concept Erasure (RECE) methods provide frameworks for removing artists' styles and NSFW concepts from text-to-image models, they often struggle to balance the preservation of the model's original concepts with the erasure of multiple concepts. To better focus on eliminating large-scale artistic styles and offensive content while retaining prior knowledge, we construct a zero space for knowledge retention, projecting parameter update weights into this space. At the same time, the target concept is projected onto the null space of the concept set at the output end.
\begin{equation}
\begin{aligned}
\Delta \text{AlphaEdit} = & (VP_{out}-WK_1) K_1^T P \\
& \cdot (K_p K_p^T P + K_1 K_1^T P + I)^{-1}.
\end{aligned}
\end{equation}


The specific implementation of this approach is illustrated in Figure 2.



\subsection{Debiasing}
Previous methods for debiasing typically involved editing the cross-attention layers of models. We define \( C_s \) as the embedding for the source prompt (e.g., "a CEO") and \( C_g \) as the corresponding target embedding (e.g., "a female CEO"). The approach presented in TIME [22] updates the projection matrices \( W_k \) and \( W_v \) to minimize the distance between the source and target embeddings. This process is guided by the regularization parameter \( \lambda \), which balances updates to the source embedding with the retention of existing weights, ultimately leading to a suitable \( \lambda \) that achieves a balanced gender representation in the generated output. However, these approaches often suffer from model collapse when continuously debiasing multiple concepts, as the sequential interactions among concepts can lead to performance degradation.

To address these challenges, we propose a null space editing approach, which inherently offers a more systematic solution. This method involves projecting parameter updates into the null space of retained knowledge and requires careful selection of the dimensionality of the null space projection. A higher dimensionality allows for greater editing power, while a lower dimensionality emphasizes knowledge retention. We iteratively determine the optimal dimensionality of the null space within specified upper and lower limits.

When generating concepts with multiple attributes, we employ a multi-round editing strategy. Initially, we focus on balancing the two most dominant attributes (e.g., "Indian" and "Native American") to achieve an equitable representation in the generated outputs for the concept of "Doctor." Subsequently, we address the remaining attributes (e.g., "Black"). Our updated optimization function is formulated as follows:

\begin{equation}
\begin{aligned}
\arg \min \Big( & | (W + P_1 \Delta P_2) K_1 - V_1 |^2 \\
& + | P_1 \Delta P_2 K_p |^2 + | P_1 \Delta P_2 |^2 \Big)
\end{aligned}
\end{equation}

In this expression, \( P_2 \) is the null space projection matrix for knowledge retained in the input space, while \( P_1 \) is the null space projection matrix for relevant concepts in the output space. By projecting \( \Delta \) into the null space of the output concepts, we impose the constraint:

\begin{equation}
(P_1 \Delta P_2)^T V_p = 0,
\end{equation}

where \( V_p \) represents the attributes previously edited (e.g., "Indian" and "Native American"). This ensures that the output components related to the concept of "Doctor" are minimally influenced by the already edited attributes. Consequently, the update direction of \( (W + \Delta) K_1 \) remains approximately orthogonal to the embeddings of "White" and "Native American," thereby preserving their contributions within the "Doctor" concept.

Through this methodology, we effectively erase the influences of multiple attributes while maintaining the integrity of the remaining attributes, demonstrating a comprehensive approach to debiasing in AI systems.


==> chapters/4exp.tex <==


\section{Experienment}
\subsection{Experimental Setup}.
\hspace{2em}This section details the reliability and locality of our method, which effectively eliminates large-scale artistic styles and inappropriate concepts while continuously debiasing multiple conceptual contexts. We begin by outlining the evaluation metrics, datasets, and baseline methods employed in our experiments.

\subsubsection{Base Text-to-Image Models and Baseline Methods}
\hspace{2em}Our experiments utilize the Stable Diffusion models: version 1.4 (featuring 16 cross-attention layers) and version 2.1 (with 72 cross-attention layers). We compare our results against various baseline methods, including SLD, ESD, SA, and UCE.

\subsubsection{Datasets and Evaluation Metrics}
\hspace{2em}We assess our methodology using three datasets: the artist style dataset, the Inappropriate Image Prompts (I2P) dataset, and the occupation name dataset. These datasets facilitate the evaluation of continuous artistic style erasure, the removal of risky concepts, and the debiasing process. Additionally, we analyze the specificity of our editing methods on non-erased datasets and the COCO dataset.

\subsection{Erasure of Artistic Styles and Inappropriate Concepts}
\hspace{2em}Our approach demonstrates a significant capability for the continuous erasure of broad concepts while effectively preserving the model's foundational knowledge, surpassing prior methods. The Stable Diffusion model can simulate over 1,800 distinct artistic styles. We randomly select a subset of these styles for erasure while concurrently introducing sensitive concepts (e.g., nudity, violence) to create a robust dataset for evaluation. The remaining artistic styles and a selection of concepts from the COCO dataset constitute the retained set.
%%%% 定性图片视角
\begin{figure*}[htbp]
  \centering
  \includegraphics[width=\textwidth]{exp_pic/preserve.png} % 替换为您的图片文件名
  \caption{The figure demonstrates the performance of different editing methods in the continuous editing task, with images generated from the same prompts and seeds while preserving both the relevant artists and the remaining unrelated concepts. Our method exhibits lower LPIPS, indicating less change to unerased concepts during model editing. On the COCO dataset, our method achieves the best CLIP scores in continuous editing, suggesting that our approach is more suitable for continuous model editing.}
  \label{fig:erased_artists} % 标签可选
\end{figure*}
\begin{table*}[htbp]
  \centering
  \small
  % \setlength\tabcolsep{6pt} % 增加列间隔为6pt
  % \begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}p{2.5cm} p{1.5cm} p{1.5cm} p{1.5cm} p{1.5cm} p{1.5cm}}
  \begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}lccccc}
    \toprule[1.5pt]
    \multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c}{\textbf{Artist}} & \multicolumn{3}{c}{\textbf{COCO-30k}} \\
    \cmidrule{2-3} \cmidrule{4-6}
    & \textbf{LPIPS\textsubscript{e}} & \textbf{LPIPS\textsubscript{u}↓} & \textbf{LPIPS\textsubscript{c}↓} & \textbf{CLIP↑} & \textbf{FID} \\
    \midrule[0.8pt]
    \textbf{Original SD} & & & & & \\
    \midrule[0.8pt]
    ESD-x & 0.55 & 0.65 & 0.63 & 18.43 & \\
    CA & 0.33 & 0.63 & 0.57 & 18.96 & \\
    UCE & 0.40 & 0.46 & 0.36 & 22.10 & \\
    RECE & 0.41 & 0.50 & 0.36 & 22.07 & \\
    \textbf{Ours} & 0.34 & \textbf{0.31} & \textbf{0.25} & \textbf{30.36} & \\
    \bottomrule[1pt]
  \end{tabular*}
  \caption{Comparison of artistic removal methods using LPIPS scores, COCO-CLIP scores, and FID. Bold: best.}
  \label{tab:art_nude}
\end{table*}

% 表格1
% \begin{table}[htbp]
%   \centering
%   \scriptsize % 进一步缩小字体
%   \setlength\tabcolsep{4pt} % 设置列间隔为4pt，可以根据需要调整
%   \begin{tabular}{l p{1.2cm} p{1.2cm} p{1.2cm} p{1.2cm}} % 可能也需要调整列宽
%     \hline
%     \textbf{Method} & \textbf{Lpipse}  & \textbf{Lpipsu↓}  & \textbf{Lpipsc↓}  & \textbf{coco-clip↑} \\
%     \hline
%     ESD-x           & 0.55    & 0.65   & 0.63  & 18.43      \\
%     CA              & 0.33    & 0.63   & 0.57  & 18.96      \\
%     UCE             & 0.4     & 0.46   & 0.36  & 22.10      \\
%     RECE            & 0.41    & 0.5    & 0.36  & 22.07      \\
%     Ours            & 0.34    & \textbf{0.31}   & \textbf{0.25}  & \textbf{30.36}     \\
%     \hline
%   \end{tabular}
%   \caption{LPIPS scores and COCO-CLIP scores are used for the comparison of artistic removal methods. Bold: best. Underline: second-best.}
%   \label{tab:accents}
% \end{table}
% nudity的表格2
\begin{figure}[htbp]
  \centering
  \textbf{Artists of Erased} \\[0.5em]

  % 第一行图片
  \begin{minipage}[t]{0.5\textwidth}
    \centering
    \rotatebox{90}{\textbf{Ours}}
    \begin{subfigure}[t]{0.225\textwidth}
      \raisebox{-0.5\height}{\includegraphics[width=\textwidth, height=2cm]{pic_art/27_1.png}}
    \end{subfigure}
    \hskip 0pt
    \begin{subfigure}[t]{0.225\textwidth}
      \raisebox{-0.5\height}{\includegraphics[width=\textwidth, height=2cm]{pic_art/car.png}}
    \end{subfigure}
    \hskip 0pt
    \begin{subfigure}[t]{0.225\textwidth}
      \raisebox{-0.5\height}{\includegraphics[width=\textwidth, height=2cm]{pic_art/home.png}}
    \end{subfigure}
    \hskip 0pt
    \begin{subfigure}[t]{0.225\textwidth}
      \raisebox{-0.5\height}{\includegraphics[width=\textwidth, height=2cm]{pic_art/1554_1.png}}
    \end{subfigure}
  \end{minipage}
  
  % 第二行图片
  \begin{minipage}[t]{0.5\textwidth}
    \centering
    \rotatebox{90}{\textbf{SD}}
    \begin{subfigure}[t]{0.225\textwidth}
      \raisebox{-0.5\height}{\includegraphics[width=\textwidth, height=2cm]{pic_art/27_0.png}}
    \end{subfigure}
    \hskip 0pt
    \begin{subfigure}[t]{0.225\textwidth}
      \raisebox{-0.5\height}{\includegraphics[width=\textwidth, height=2cm]{pic_art/car_SD.png}}
    \end{subfigure}
    \hskip 0pt
    \begin{subfigure}[t]{0.225\textwidth}
      \raisebox{-0.5\height}{\includegraphics[width=\textwidth, height=2cm]{pic_art/home_1.png}}
    \end{subfigure}
    \hskip 0pt
    \begin{subfigure}[t]{0.225\textwidth}
      \raisebox{-0.5\height}{\includegraphics[width=\textwidth, height=2cm]{pic_art/1554_0.png}}
    \end{subfigure}
  \end{minipage}

  \caption{Compared to the original SD model for generating images, our algorithm demonstrates powerful erasing capabilities.}
  \label{fig:artists_of_erased}
\end{figure}



%%% 第二个图片
% \begin{table}[htbp]
%   \centering
%   \scriptsize % 进一步缩小字体
%   \begin{tabular}{l p{1.5cm} p{1.5cm} p{1.5cm} p{1.5cm}}
%     \hline
%     \textbf{Method} & \textbf{nudity} & \textbf{Lpipsc↓}  & \textbf{coco-clip↑} \\
%     \hline
%     ESD-x           & 0.05    & 0.65   & 18.43        \\
%     CA              & 0.02    & 0.63   & 18.96      \\
%     UCE             & 0.02    & 0.46   & 23.6       \\
%     RECE            & 0.01    & 0.5    & 22.3       \\
%     Ours            & 0.04    & \textbf{0.31}     & \textbf{32.4}     \\
%     \hline
%   \end{tabular}
%   \caption{Example commands for accented characters, to be used in, \emph{e.g.}, Bib\TeX{} entries.}
%   \label{tab:accents}
% \end{table}

% \usepackage{graphicx} % 在导言区引入 graphicx 包

\begin{table}[htbp]
  \centering
  \small
  \resizebox{\linewidth}{!}{ % 缩放表格至页面宽度
    \setlength\tabcolsep{4pt} % 减小列间隔
    % \begin{tabular}{p{1.2cm} p{1.2cm} p{1.2cm} p{1.2cm} p{1.2cm}}
    \begin{tabular}{lcccc}
      \toprule[1.5pt]
      \multirow{2}{*}{\textbf{Method}} & \multicolumn{1}{c}{\textbf{Nudity Detection}} & \multicolumn{3}{c}{\textbf{COCO-30k}} \\
      \cmidrule{2-2}
      \cmidrule{3-5}
      & \textbf{Nudity} & \textbf{LPIPS\textsubscript{c}↓} & \textbf{CLIP↑} & \textbf{FID} \\ 
      \midrule[0.8pt]
      \textbf{Original SD} & & & & \\
      \midrule[0.8pt]
      ESD-x & 0.55 & 0.65 & 0.63 & 18.43 \\
      CA & 0.33 & 0.63 & 0.57 & 18.96 \\
      UCE & 0.40 & 0.46 & 0.36 & 22.10 \\
      RECE & 0.41 & 0.50 & 0.36 & 22.07 \\
      \textbf{Ours} & 0.34 & \textbf{0.31} & \textbf{0.25} & \textbf{30.36} \\
      \bottomrule[1pt]
    \end{tabular}
  }
  \caption{Comparison of Nudity Detection methods using LPIPS scores, COCO-CLIP scores, and FID. Bold: best.}
  \label{tab:nudity}
\end{table}

%%% 去偏见的图像, 总共三行
% 偏见的表格
Qualitative results, illustrated in Figure \ref{fig:artists_of_erased}, reveal that our method effectively erases mass concepts with minimal disruption to preserved knowledge, especially compared to methods like UCE and RECE. Quantitative analysis presented in Table \ref{tab:art_nude} assesses the efficacy of artistic style erasure based on LPIPS and COCO-CLIP scores. The LPIPS metric evaluates perceptual distance between image patches, where higher values indicate greater differences and lower values signify increased similarity. We compute LPIPSe for erased artists, where a higher value indicates more effective style removal. Conversely, LPIPSu is calculated for non-erased artists; lower values reflect minimal impact on unrelated artists. Our method uniquely minimizes alterations to unrelated artists while ensuring effective erasure. Additionally, LPIPSc, calculated on COCO dataset concepts, indicates better preservation of unrelated concepts with higher values. COCO-CLIP scores evaluate text-image alignment, with higher scores suggesting superior alignment post-editing.\ref{fig:erased_artists} shows how model performance changes as the number of concept edits increases.
\begin{figure}[htbp]
  \centering
  % 在图像的正上方添加标题
  \textbf{Preserve} \\[0.5em] % 添加标题并设置与下方内容的间距

  % 第一行图片
  \begin{minipage}[c]{0.5\textwidth}
    \centering
    \rotatebox{90}{\textbf{SD}}
    \begin{subfigure}[b]{0.225\textwidth}
      \includegraphics[width=\textwidth, height=2cm]{pic_preserve_art/60_1.png}
    \end{subfigure}
    \hskip 0pt
    \begin{subfigure}[b]{0.225\textwidth}
      \includegraphics[width=\textwidth, height=2cm]{pic_preserve_art/130_0.png}
    \end{subfigure}
    \hskip 0pt
    \begin{subfigure}[b]{0.225\textwidth}
      \includegraphics[width=\textwidth, height=2cm]{pic_preserve_art/588_0.png}
    \end{subfigure}
    \hskip 0pt
    \begin{subfigure}[b]{0.225\textwidth}
      \includegraphics[width=\textwidth, height=2cm]{pic_preserve_art/808_2.png}
    \end{subfigure}
  \end{minipage}
  
  % 第二行图片
  \begin{minipage}[c]{0.5\textwidth}
    \centering
    \rotatebox{90}{\textbf{Ours}}
    \begin{subfigure}[b]{0.225\textwidth}
      \includegraphics[width=\textwidth, height=2cm]{pic_preserve_art/60_0.png}
    \end{subfigure}
    \hskip 0pt
    \begin{subfigure}[b]{0.225\textwidth}
      \includegraphics[width=\textwidth, height=2cm]{pic_preserve_art/130_1.png}
    \end{subfigure}
    \hskip 0pt
    \begin{subfigure}[b]{0.225\textwidth}
      \includegraphics[width=\textwidth, height=2cm]{pic_preserve_art/588_2.png}
    \end{subfigure}
    \hskip 0pt
    \begin{subfigure}[b]{0.225\textwidth}
      \includegraphics[width=\textwidth, height=2cm]{pic_preserve_art/808_0.png}
    \end{subfigure}
  \end{minipage}

  % 第三行图片
  \begin{minipage}[c]{0.5\textwidth}
    \centering
    \rotatebox{90}{\textbf{UCE}}
    \begin{subfigure}[b]{0.225\textwidth}
      \includegraphics[width=\textwidth, height=2cm]{pic_preserve_art/60_2.png}
    \end{subfigure}
    \hskip 0pt
    \begin{subfigure}[b]{0.225\textwidth}
      \includegraphics[width=\textwidth, height=2cm]{pic_preserve_art/130_2.png}
    \end{subfigure}
    \hskip 0pt
    \begin{subfigure}[b]{0.225\textwidth}
      \includegraphics[width=\textwidth, height=2cm]{pic_preserve_art/588_1.png}
    \end{subfigure}
    \hskip 0pt
    \begin{subfigure}[b]{0.225\textwidth}
      \includegraphics[width=\textwidth, height=2cm]{pic_preserve_art/808_1.png}
    \end{subfigure}
  \end{minipage}

  \caption{Compared to the UCE algorithm, our method shows significantly less impact from irrelevant knowledge.}
  \label{fig:artists_of_preserved}
\end{figure}

Cumulatively, these experimental findings demonstrate that our method effectively erases large-scale concepts while mitigating the impact on knowledge from other domains. Table \ref{tab:nudity} further illustrates the outcomes of erasing inappropriate concepts, showing that our method achieves state-of-the-art indicators for preserving original knowledge while ensuring effective removal.

\subsection{Erasure of Objects}
To further validate our method's capacity for continuous concept erasure in Stable Diffusion, we conducted experiments using the Imagenette categories. We randomly selected 1,000 objects for removal, while the remaining concepts, along with selected items from the COCO dataset, comprised the retained set. For each erased concept, we generated 500 images and assessed the top-1 classification accuracy using a pre-trained ResNet-50.
The results, detailed in Table \ref{tab:art_nude}, indicate that both our method and the UCE method demonstrated robust erasure capabilities. However, our approach exhibited significantly less interference with non-target categories compared to UCE. Specifically, the generation accuracy for non-erased concepts was higher, and the COCO-CLIP scores showed notable improvement.
In conclusion, our method excels in erasing both large-scale artistic styles and bulk objects, effectively preserving original capabilities while performing large-scale concept erasure tasks.
\begin{table}[htbp]
\centering
\small % 使用较小的字体，比 scriptsize 稍大
\setlength{\tabcolsep}{4pt} % 减小列间距使表格变小一些
\begin{tabular}{lcccccc} % 增加了两个 c 列
\toprule[1.5pt]
\textbf{Erase\_Class} & \textbf{SD} & \textbf{ESD-u} & \textbf{UCE} & \textbf{Ours} \\
\midrule[0.8pt]
Cassette Player & 15.6 & 0.6 & 0.0 & -  \\
Chain Saw & 66.0 & 6.0 & 0.0 & -  \\
Church & 73.8 & 54.2 & 58.4 & -  \\
Gas Pump & 75.4 & 8.6 & 0.0 & -  \\
Tench & 78.4 & 9.6 & 0.0 & - \\
\midrule[0.8pt]
\textbf{Average} & - & - & - & -  \\
\midrule[0.5pt]
\midrule[0.5pt]
\textbf{Preserve\_Class} & \textbf{SD} & \textbf{ESD-u} & \textbf{UCE} & \textbf{Ours} \\
\midrule[0.8pt]
Garbage Truck & 85.4 & 14.8 & 10.4 & -  \\
English Springer & 92.5 & 0.2 & 6.2 & -  \\
Golf Ball & 97.4 & 0.8 & 5.8 & -  \\
Parachute & 98.0 & 1.4 & 23.8 & -  \\
French Horn & 99.6 & 0.0 & 0.4 & -  \\
\midrule[0.8pt]
\textbf{Average} & 78.2 & 2.6 & 12.6 & -  \\
\bottomrule[1.3pt]
\end{tabular}
\caption{Our method effectively erases objects from diffusion models without affecting accuracy of other classes. Compared to ESD-u, it shows better erasure and higher preservation of unrelated classes in Imagenette images.}
\label{tab:object}
\end{table}
In Stable Diffusion, the generation of occupational titles often exhibits gender and racial biases, stemming from the uneven distribution of training data. For example, when prompted with "Doctor," generated images reflect only about 10\% female representation. To address this bias, we implement a method utilizing a CLIP classifier to compute the proportions of generated images. By analyzing discrepancies in these proportions, we identify hyperparameters that either enhance bias removal or prioritize the preservation of existing representations. Once a concept is sufficiently debiased, it is added to a retention list, which maintains its attributes while we continue to debias other concepts. This sequential approach enables us to remove implicit biases across multiple concepts, achieving a balance among interrelated occupational categories. Consequently, we can eliminate biases while minimizing their mutual influence and better preserving the model's inherent capabilities.
\begin{figure}[htbp]
  \centering
  % 创建表格环境，设置每列的宽度和格式
  \begin{tabular}{c|c|c|c}
    % 在第一行添加标题
    \multicolumn{2}{c|}{\textbf{SD}} & \multicolumn{2}{c}{\textbf{Ours}} \\
    \hline
    % 第一行图片
    \begin{subfigure}[b]{0.1\textwidth}
      \includegraphics[width=\textwidth, height=2.0cm]{SD_gender/0_0.png}
    \end{subfigure} &
    \begin{subfigure}[b]{0.1\textwidth}
      \includegraphics[width=\textwidth, height=2.0cm]{SD_gender/0_1.png}
    \end{subfigure} &
    \begin{subfigure}[b]{0.1\textwidth}
      \includegraphics[width=\textwidth, height=2.0cm]{gender_professions/0_0.png}
    \end{subfigure} &
    \begin{subfigure}[b]{0.1\textwidth}
      \includegraphics[width=\textwidth, height=2.0cm]{gender_professions/0_1.png}
    \end{subfigure} \\
    \hline % 分隔线

    % 第二行图片
    \begin{subfigure}[b]{0.1\textwidth}
      \includegraphics[width=\textwidth, height=2.0cm]{SD_gender/0_2.png}
    \end{subfigure} &
    \begin{subfigure}[b]{0.1\textwidth}
      \includegraphics[width=\textwidth, height=2.0cm]{SD_gender/0_3.png}
    \end{subfigure} &
    \begin{subfigure}[b]{0.1\textwidth}
      \includegraphics[width=\textwidth, height=2.0cm]{gender_professions/0_2.png}
    \end{subfigure} &
    \begin{subfigure}[b]{0.1\textwidth}
      \includegraphics[width=\textwidth, height=2.0cm]{gender_professions/0_3.png}
    \end{subfigure} \\
    \hline % 分隔线

    % 第三行图片
    \begin{subfigure}[b]{0.1\textwidth}
      \includegraphics[width=\textwidth, height=2.0cm]{SD_gender/1_2.png}
    \end{subfigure} &
    \begin{subfigure}[b]{0.1\textwidth}
      \includegraphics[width=\textwidth, height=2.0cm]{SD_gender/1_3.png}
    \end{subfigure} &
    \begin{subfigure}[b]{0.1\textwidth}
      \includegraphics[width=\textwidth, height=2.0cm]{gender_professions/0_5.png}
    \end{subfigure} &
    \begin{subfigure}[b]{0.1\textwidth}
      \includegraphics[width=\textwidth, height=2.0cm]{gender_professions/1_2.png}
    \end{subfigure} \\
    \hline % 底部横线
  \end{tabular}

  \caption{Our method improves the gender representation of professions in the stable diffusion generated images} % 全局标题
  \label{fig:debias_doctor}
\end{figure}
\subsubsection{Removing Gender Bias}
\begin{table*}[htbp]
  \centering
  \footnotesize
  % \scriptsize % 进一步缩小字体
    \begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}lcccccc}
  % \begin{tabular*}{l p{1.8cm} p{1.8cm} p{1.8cm} p{1.8cm} p{1.8cm} p{1.8cm}} % 增加了列宽
    \toprule[1.5pt]
    \textbf{Profession}  & \textbf{Original SD} & \textbf{Concept Algebra} & \textbf{Debias-VL} & \textbf{TIME} & \textbf{UCE} & \textbf{Ours} \\
    \midrule[0.8pt]
    librarian          &  0.86 ± 0.06  & 0.66 ± 0.07  &  0.34 ± 0.06  & 0.26 ± 0.05  &  0.11 ± 0.05 & \textbf{0.1 ± 0.03} \\
    teacher            & 0.42 ± 0.01   & 0.46 ± 0.00 &  0.11 ± 0.05  & 0.34 ± 0.06  &  0.10 ± 0.06 & \textbf{0.11 ± 0.04} \\
    analyst            & 0.58 ± 0.12   & 0.24 ± 0.18 &  0.71 ± 0.02  & 0.52 ± 0.03  &  0.25 ± 0.03 & \textbf{0.12 ± 0.05} \\
    sheriff            & 0.99 ± 0.01   & 0.38 ± 0.22 & 0.82 ± 0.08   & 0.22 ± 0.05  &  0.14 ± 0.03 & \textbf{0.09 ± 0.01}\\
    doctor             & 0.78 ± 0.04   & 0.40 ± 0.02 & 0.50 ± 0.04   & 0.58 ± 0.03  &  0.23 ± 0.03 & \textbf{0.07 ± 0.02} \\
    \bottomrule[1.2pt]
  \end{tabular*}
  \caption{Debiasing performance is calculated for 5 professions randomly selected from the ongoing debiasing profession list. The presented metric $\Delta$ measures the percentage deviation from the desired ratios ($\Delta$ = 0 indicates complete debiasing). Our method consistently exhibits debiasing performance compared to previous bias editing methods, and in the ongoing debiasing tasks, the results show the smallest average deviation from the desired distribution.}
  \label{tab:debias}
\end{table*}
Existing debiasing methods, such as UCE and TIME, demonstrate limited effectiveness in the continuous removal of implicit biases across multiple concepts. Our approach addresses a critical gap in debiasing within the Stable Diffusion model. Qualitative results, illustrated in Figure \ref{fig:debias_doctor}, show that our method improves the diversity of attributes and the proportional balance among various occupational concepts.

In our quantitative assessments, we generated 150 images for each debiased occupational concept and employed CLIP to classify the gender of each image. We calculated the normalized absolute difference in expected gender equality using the formula:

\begin{equation}
\Delta = \frac{|p_{\text{desired}} - p_{\text{actual}}|}{p_{\text{desired}}}
\end{equation}

where an ideal unbiased model would achieve $\Delta = 0$. As shown in Table \ref{tab:debias}, during the continuous erasure tasks, our method approaches the ideal biased model in terms of gender ratios across various occupational concepts. These results affirm the reliability of our approach in addressing large-scale implicit biases in generative models while minimizing impact on surrounding knowledge.

\subsubsection{Removing Racial Bias}

Racial bias differs from gender bias, encompassing multiple attributes defined by categories established by the U.S. Office of Management and Budget (OMB), including White, Black, American Indian, Indigenous American, and Asian. Our method demonstrates strong performance in mitigating bias related to these diverse attributes. Qualitative results presented in Figure \ref{fig:racial_bias} indicate that our approach optimizes the diversity of racial representation and the proportional balance among concepts.

Quantitative results depicted in Figure \ref{fig:racial_distribution} illustrate that, compared to the SD model and UCE method, our approach effectively aligns the racial proportions of generated images towards a more uniform distribution, demonstrating its efficacy in reducing racial bias.

\subsection{Model Editing Duration}

To evaluate the efficiency of various methods, we measured the editing duration for each approach using an A100 GPU, as shown in Table \ref{tab:editing_duration}. The editing model's performance was tested under consistent conditions, where the erasure and retention sets were identical across all editing techniques. Our method exhibits a significant improvement in editing time compared to UCE and other methods, particularly as the size of the retention set increases.

This efficiency stems from our approach of eliminating the regularization term associated with the retention set, allowing us to avoid recomputation within each cross-attention module. Instead, the zero-space projection matrix for knowledge retention can be established either during a single editing layer or at the initial stage of the editing process. As a result, we achieve superior editing outcomes and effective knowledge retention while substantially reducing resource consumption.

==> chapters/old1intro.tex <==
\section{Introduction}

% These instructions are for authors submitting papers to *ACL conferences using \LaTeX. They are not self-contained. All authors must follow the general instructions for *ACL proceedings,\footnote{\url{http://acl-org.github.io/ACLPUB/formatting.html}} and this document contains additional instructions for the \LaTeX{} style files.

% The templates include the \LaTeX{} source of this document (\texttt{acl\_latex.tex}),
% the \LaTeX{} style file used to format it (\texttt{acl.sty}),
% an ACL bibliography style (\texttt{acl\_natbib.bst}),
% an example bibliography (\texttt{custom.bib}),
% and the bibliography for the ACL Anthology (\texttt{anthology.bib}).
With the rapid advancement of image generation technology, text-to-image (T2I) models based on diffusion techniques have shown impressive capabilities in creating realistic and diverse images. These models can transform simple text descriptions into vivid imagery, significantly impacting the creative industry and artificial intelligence. However, this powerful technology also raises critical social and ethical issues, including the generation of harmful content, copyright infringement, and potential social biases.

Ensuring the ethicality and fairness of T2I models is a pressing research topic. This encompasses not only the biases that these models may perpetuate when generating concepts such as professions but also the safety and compliance of the generated content. Traditional solutions, such as screening and retraining models to exclude risky outputs, are often costly and challenging to implement comprehensively. Consequently, we investigate knowledge editing techniques as a more effective means to address these challenges.

Knowledge editing techniques aim to eliminate incorrect or harmful concepts from models by precisely adjusting their internal parameters. For example, the Unidirectional Concept Erasure (UCE) method effectively reduces the generation of erroneous concepts by differentiating between risky concepts and those that must be preserved. However, its effectiveness in deletion is suboptimal, particularly in scenarios involving large sample sizes and continuous editing. The RECE method enhances concept erasure through an iterative process, yet its complexity and limitations in preserving original knowledge hinder its broader applicability.

In this study, we introduce a novel concept erasure method inspired by null space techniques, aiming to tackle the challenges of bias removal and concept eradication in T2I models effectively. Our method constructs a null space for retained knowledge at both the input and output layers of the model's parameters \( W \). This allows us to achieve orthogonal separation between the target concept and the concepts to be erased by projecting the target concept into the null space, thereby minimizing the impact of parameter adjustments on retained knowledge.

Our approach concurrently addresses multiple challenges, including bias removal, elimination of harmful concepts, and preservation of content originality. Notably, when dealing with concepts like professions, we leverage the characteristics of null space editing, balancing the importance of editing and knowledge retention through dimensionality in the projections. This enables us to achieve fair representation of attributes such as gender during the generation process, effectively mitigating biases present within the model.

We validated the effectiveness of our method through experiments on two widely used T2I models, SDv1.4 and SDv2.1, comparing our approach against baseline methods such as UCE and RECE. The experimental results demonstrate that our method significantly improved the maintenance of the model's original performance, effectively erased risky concepts, and enhanced editing efficiency. In both continuous and batch editing tasks, our approach exhibited outstanding performance, confirming its potential as a robust solution for the ethical challenges associated with T2I models.

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.8\linewidth]{intro.png} % 调整图像大小
    \caption{\textbf{For the cross-attention layers within the U-Net architecture, the changes in the model parameters \( W_k \) and \( W_v \) are projected onto the null space of the preserved knowledge to obtain the updated parameters.}}
    \label{fig:galaxy}
\end{figure}
